Feedback Prediction for Proactive HARQ in the Context of Industrial Internet of Things

In this work, we investigate proactive Hybrid Automatic Repeat reQuest (HARQ) using link-level simulations for multiple packet sizes, modulation orders, BLock Error Rate (BLER) targets and two delay budgets of 1 ms and 2 ms, in the context of Industrial Internet of Things (IIOT) applications. In particular, we propose an enhanced proactive HARQ protocol using a feedback prediction mechanism. We show that the enhanced protocol achieves a significant gain over the classical proactive HARQ in terms of energy efficiency for almost all evaluated BLER targets at least for sufficiently large feedback delays. Furthermore, we demonstrate that the proposed protocol clearly outperforms the classical proactive HARQ in all scenarios when taking a processing delay reduction due to the less complex prediction approach into account, achieving an energy efficiency gain in the range of 11% up to 15% for very stringent latency budgets of 1 ms at $10^{-2}$ BLER and from 4% up to 7.5% for less stringent latency budgets of 2 ms at $10^{-3}$ BLER. Furthermore, we show that power-constrained proactive HARQ with prediction even outperforms unconstrained reactive HARQ for sufficiently large feedback delays.

==> acro.definitions.tex <==
% --------------------------------------------------------------------------
% the ACRO package
% 
%   Typeset Acronyms
% 
% --------------------------------------------------------------------------
% Clemens Niederberger
% Web:    https://bitbucket.org/cgnieder/acro/
% E-Mail: contact@mychemistry.eu
% --------------------------------------------------------------------------
% Copyright 2011--2020 Clemens Niederberger
% 
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% 
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is Clemens Niederberger.
% --------------------------------------------------------------------------
% The acro package consists of the files
% - acro.sty, acro.definitions.tex, acro.cfg
% - acro-manual.tex, acro-manual.pdf, acro-manual.cls
% - acro.history, README
% --------------------------------------------------------------------------
% If you have any ideas, questions, suggestions or bugs to report, please
% feel free to contact me.
% --------------------------------------------------------------------------
\ExplSyntaxOn

% document commands:
\NewDocumentCommand \DeclareAcronym {mm}
  { \acro_declare_acronym:nn {#1} {#2} }

\NewDocumentCommand \acsetup { m }
  {
    \tl_if_blank:nF {#1}
      { \keys_set:nn {acro} {#1} }
    \ignorespaces
  }

\NewDocumentCommand \ProvideAcroEnding {mmm}
  { \acro_provide_ending:nnn {#1} {#2} {#3} }

\NewDocumentCommand \AcroRegisterTrailing {mm}
  { \acro_register_trailing_token:Nn #1 {#2} }

\NewDocumentCommand \DeclareAcroTranslation {mm}
  { \acro_declare_translation:nn {#1} {#2} }

\DeclareExpandableDocumentCommand \acifused { m }
  { \acro_if_acronym_used:nTF {#1} }

\NewDocumentCommand \acresetall {}
  { \acro_reset_all: }

\NewDocumentCommand \acuseall {}
  { \acro_mark_all_as_used: }

\NewDocumentCommand \acreset { > { \SplitList {,} } m }
  { \ProcessList {#1} { \acro_reset:n } \ignorespaces }

\NewDocumentCommand \acuse { > { \SplitList {,} } m }
  { \ProcessList {#1} { \acro_mark_as_used:n } \ignorespaces }

\NewDocumentCommand \acfirstupper {m}
  { \acro_first_upper_case:n {#1} }

\NewExpandableDocumentCommand \aciffirst {+m+m}
  { \bool_if:NTF \l__acro_first_instance_bool {#1} {#2} }

\NewDocumentCommand \acdot   {} { \acro_dot: }
\NewDocumentCommand \acspace {} { \acro_space: }

\NewDocumentCommand \acbarrier {}
  { \acro_barrier: }

\NewDocumentCommand \acswitchoff {}
  { \acro_switch_off: }

\NewDocumentCommand \acswitchon {}
  { \acro_switch_on: }

\NewDocumentCommand \printacronyms { O{} }
  { \acro_print_acronyms:n {#1} }

% --------------------------------------------------------------------------
% styles
% #1: name
% #2: template
% #3: settings
\NewDocumentCommand \DeclareAcroFirstStyle {mmm}
  { \acro_declare_first_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroExtraStyle {mmm}
  { \acro_declare_extra_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroPageStyle {mmm}
  { \acro_declare_page_style:nnn {#1} {#2} {#3} }

\NewDocumentCommand \DeclareAcroListHeading {mm}
  { \acro_declare_list_heading:nn {#1} {#2} }

\NewDocumentCommand \DeclareAcroListStyle {mmm}
  { \acro_declare_list_style:nnn {#1} {#2} {#3} }

% --------------------------------------------------------------------------
% endings:
\ProvideAcroEnding {plural} {s} {s}

% --------------------------------------------------------------------------
% use acronyms:
% automatic:
\NewAcroCommand \ac
  { \acro_use:n {#1} }

\NewAcroCommand \Ac
  {
    \acro_first_upper:
    \acro_use:n {#1}
  }

\NewAcroCommand \iac
  {
    \acro_indefinite:
    \acro_use:n {#1}
  }

\NewAcroCommand \Iac
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_use:n {#1}
  }

\NewAcroCommand \acp
  {
    \acro_plural:
    \acro_use:n {#1}
  }

\NewAcroCommand \Acp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_use:n {#1}
  }

\NewAcroCommand \acsingle
  {
    \acro_get:n {#1}
    \acro_single:n {#1}
  }

\NewAcroCommand \acpsingle
  {
    \acro_get:n {#1}
    \acro_plural:
    \acro_single:n {#1}
  }

\NewAcroCommand \Acsingle
  {
    \acro_get:n {#1}
    \acro_first_upper:
    \acro_single:n {#1}
  }

\NewAcroCommand \Acpsingle
  {
    \acro_get:n {#1}
    \acro_first_upper:
    \acro_plural:
    \acro_single:n {#1}
  }

% short:
\NewAcroCommand \acs
  { \acro_short:n {#1} }

\NewAcroCommand \Acs
  {
    \acro_first_upper:
    \acro_short:n {#1}
  }

\NewAcroCommand \iacs
  {
    \acro_indefinite:
    \acro_short:n {#1}
  }

\NewAcroCommand \Iacs
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_short:n {#1}
  }

\NewAcroCommand \acsp
  {
    \acro_plural:
    \acro_short:n {#1}
  }

\NewAcroCommand \Acsp
  {
    \acro_first_upper:
    \acro_plural:
    \acro_short:n {#1}
  }

% alt:
\NewAcroCommand \aca
  { \acro_alt:n {#1} }

\NewAcroCommand \Aca
  {
    \acro_first_upper:
    \acro_alt:n {#1}
  }
  
\NewAcroCommand \iaca
  {
    \acro_indefinite:
    \acro_alt:n {#1}
  }

\NewAcroCommand \Iaca
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_alt:n {#1}
  }

\NewAcroCommand \acap
  {
    \acro_plural:
    \acro_alt:n {#1}
  }

\NewAcroCommand \Acap
  {
    \acro_first_upper:
    \acro_plural:
    \acro_alt:n {#1}
  }

% long:
\NewAcroCommand \acl
  { \acro_long:n {#1} }

\NewAcroCommand \Acl
  {
    \acro_first_upper:
    \acro_long:n {#1}
  }

\NewAcroCommand \iacl
  {
    \acro_indefinite:
    \acro_long:n {#1}
  }

\NewAcroCommand \Iacl
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_long:n {#1}
  }

\NewAcroCommand \aclp
  {
    \acro_plural:
    \acro_long:n {#1}
  }

\NewAcroCommand \Aclp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_long:n {#1}
  }

% first:
\NewAcroCommand \acf
  { \acro_first:n {#1} }

\NewAcroCommand \Acf
  {
    \acro_first_upper:
    \acro_first:n {#1}
  }

\NewAcroCommand \iacf
  {
    \acro_indefinite:
    \acro_first:n {#1}
  }

\NewAcroCommand \Iacf
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_first:n {#1}
  }

\NewAcroCommand \acfp
  {
    \acro_plural:
    \acro_first:n {#1}
  }

\NewAcroCommand \Acfp
  {
    \acro_plural:
    \acro_first_upper:
    \acro_first:n {#1}
  }

% first-like:
\NewPseudoAcroCommand \acflike
  { \acro_first_like:nn {#1} {#2} }

\NewPseudoAcroCommand \iacflike
  {
    \acro_indefinite:
    \acro_first_like:nn {#1} {#2}
  }

\NewPseudoAcroCommand \Iacflike
  {
    \acro_first_upper:
    \acro_indefinite:
    \acro_first_like:nn {#1} {#2}
  }

\NewPseudoAcroCommand \acfplike
  {
    \acro_plural:
    \acro_first_like:nn {#1} {#2}
  }

% --------------------------------------------------------------------------
% first appearance styles:
\DeclareAcroFirstStyle {default} {inline}
  { }

\DeclareAcroFirstStyle {reversed} {inline}
  { reversed = true }

\DeclareAcroFirstStyle {short} {inline}
  {
    only-short = true ,
    brackets = false
  }

\DeclareAcroFirstStyle {long} {inline}
  {
    only-long = true ,
    brackets = false
  }

\DeclareAcroFirstStyle {square} {inline}
  { brackets-type = [] }

\DeclareAcroFirstStyle {plain} {inline}
  {
    brackets = false ,
    between = --
  }

\DeclareAcroFirstStyle {plain-reversed} {inline}
  { 
    brackets = false ,
    between = -- ,
    reversed = true
  }

\DeclareAcroFirstStyle {footnote} {note}
  { }

\DeclareAcroFirstStyle {footnote-reversed} {note}
  { reversed = true }

\DeclareAcroFirstStyle {sidenote} {note}
  { note-command = \sidenote {#1} }

\DeclareAcroFirstStyle {sidenote-reversed} {note}
  {
    note-command = \sidenote {#1} ,
    reversed     = true
  }

\DeclareAcroFirstStyle {empty} {note}
  { use-note = false }

% --------------------------------------------------------------------------
% extra info appearance styles:
\DeclareAcroExtraStyle {default} {inline}
  {
    brackets     = false ,
    punct        = true ,
    punct-symbol = .
  }

\DeclareAcroExtraStyle {plain} {inline}
  {
    brackets     = false ,
    punct        = true ,
    punct-symbol =
  }

\DeclareAcroExtraStyle {paren} {inline}
  {
    brackets     = true ,
    punct        = true ,
    punct-symbol =
  }

\DeclareAcroExtraStyle {bracket} {inline}
  {
    brackets      = true ,
    punct         = true ,
    punct-symbol  = ,
    brackets-type = []
  }

\DeclareAcroExtraStyle {comma} {inline}
  {
    punct         = true,
    punct-symbol  = {,} ,
    brackets      = false
  }

% --------------------------------------------------------------------------
% page number appearance styles:
\DeclareAcroPageStyle {default} {inline}
  {
    punct = true ,
    punct-symbol = .
  }
  
\DeclareAcroPageStyle {plain}   {inline}
  { punct = false }

\DeclareAcroPageStyle {comma}   {inline}
  { punct = true }

\DeclareAcroPageStyle {paren}   {inline}
  {
    brackets=true ,
    punct-symbol = ~
  }

\DeclareAcroPageStyle {none}    {inline}
  { display = false }

% --------------------------------------------------------------------------
% list heading styles:
\DeclareAcroListHeading {part}           {\part}
\DeclareAcroListHeading {part*}          {\part*}
\DeclareAcroListHeading {chapter}        {\chapter}
\DeclareAcroListHeading {chapter*}       {\chapter*}
\DeclareAcroListHeading {addchap}        {\addchap}
\DeclareAcroListHeading {section}        {\section}
\DeclareAcroListHeading {section*}       {\section*}
\DeclareAcroListHeading {addsec}         {\addsec}
\DeclareAcroListHeading {subsection}     {\subsection}
\DeclareAcroListHeading {subsection*}    {\subsection*}
\DeclareAcroListHeading {subsubsection}  {\subsubsection}
\DeclareAcroListHeading {subsubsection*} {\subsubsection*}
\DeclareAcroListHeading {none}           {\use_none:n}

% --------------------------------------------------------------------------
% list styles:
\DeclareAcroListStyle {description} {list}
  { }

\DeclareAcroListStyle {toc} {list-of}
  { }

\DeclareAcroListStyle {lof} {list-of}
  { style = lof }

\DeclareAcroListStyle {tabular} {table}
  { table = tabular }

\DeclareAcroListStyle {longtable} {table}
  { table = longtable }

\DeclareAcroListStyle {extra-tabular} {extra-table}
  { table = tabular }

\DeclareAcroListStyle {extra-longtable} {extra-table}
  { table = longtable }

\DeclareAcroListStyle {extra-tabular-rev} {extra-table}
  {
    table   = tabular ,
    reverse = true
  }

\DeclareAcroListStyle {extra-longtable-rev} {extra-table}
  {
    table   = longtable ,
    reverse = true
  }

% --------------------------------------------------------------------------
% register some tokens to be checked for:
\AcroRegisterTrailing . {dot}
\AcroRegisterTrailing - {dash}
\AcroRegisterTrailing \babelhyphen {babel-hyphen}

\acsetup { activate-trailing-tokens = dot }

% some user macros:
\cs_new_protected:Npn \acro_dot:
  { \acro_if_trailing_tokens:nF {dot} {.\@} }

\cs_new_protected:Npn \acro_space:
  { \acro_if_trailing_tokens:nF {dash,babel-hyphen} { \c_space_tl } }

% --------------------------------------------------------------------------
% translations:
% list name
\DeclareAcroTranslation {acronym-list-name}
  {
    Fallback   = Acronyms ,
    English    = Acronyms ,
    French     = Acronymes ,
    German     = Abk\"urzungen ,
    Italian    = Acronimi ,
    Portuguese = Acr\'onimos ,
    Spanish    = Siglas ,
    Catalan    = Sigles ,
    Turkish    = K\i saltmalar
  }

% page name
\DeclareAcroTranslation {acronym-page-name}
  {
    Fallback   = p. ,
    English    = p. ,
    German     = S. ,
    Portuguese = p.
  }

% pages name
\DeclareAcroTranslation {acronym-pages-name}
  {
    Fallback   = pp. ,
    English    = pp. ,
    German     = S. ,
    Portuguese = pp.
  }

% following page
\DeclareAcroTranslation {acronym-next-page}
  {
    Fallback   = f. ,
    English    = f. ,
    German     = f. ,
    Portuguese = s.
  }

% following pages
\DeclareAcroTranslation {acronym-next-pages}
  {
    Fallback   = ff. ,
    English    = ff. ,
    German     = ff. ,
    Portuguese = ss.
  }

\file_input_stop:

